Out of the Room: Generalizing Event-Based Dynamic Motion Segmentation for Complex Scenes

Rapid and reliable identification of dynamic scene parts, also known as motion segmentation, is a key challenge for mobile sensors. Contemporary RGB camera-based methods rely on modeling camera and scene properties however, are often under-constrained and fall short in unknown categories. Event cameras have the potential to overcome these limitations, but corresponding methods have only been demonstrated in smaller-scale indoor environments with simplified dynamic objects. This work presents an event-based method for class-agnostic motion segmentation that can successfully be deployed across complex large-scale outdoor environments too. To this end, we introduce a novel divide-and-conquer pipeline that combines: (a) ego-motion compensated events, computed via a scene understanding module that predicts monocular depth and camera pose as auxiliary tasks, and (b) optical flow from a dedicated optical flow module. These intermediate representations are then fed into a segmentation module that predicts motion segmentation masks. A novel transformer-based temporal attention module in the segmentation module builds correlations across adjacent 'frames' to get temporally consistent segmentation masks. Our method sets the new state-of-the-art on the classic EV-IMO benchmark (indoors), where we achieve improvements of 2.19 moving object IoU (2.22 mIoU) and 4.52 point IoU respectively, as well as on a newly-generated motion segmentation and tracking benchmark (outdoors) based on the DSEC event dataset, termed DSEC-MOTS, where we show improvement of 12.91 moving object IoU.

==> to-do.tex <==
\section{To-do List}

Titles:
\begin{itemize}
    \item EDOS: Event-based Dynamic Object Segmentation for Autonomous Driving
    \item Event-based Dynamic Scene Segmentation for Dynamics-aware SLAM
    \item XYZ-Lens: ...
    \item Event-based ... with application in Robot Perception
    \item Event-based ... for Dynamic Object Removal
    \item Event-based ... for Dynamic Scene Segmentation and SLAM
    \item Something flashy? Super low latency ...
\end{itemize}

story: event dynamics filter.
Why relevant
- How it improves map quality
- How it improves state estimation quality

(best possible) Filter plus application to SLAM. Ablating the different design choices in the motion filter.

SLAM side:
projecting from camera to LiDAR and evaluation of accuracy.

Compare motion compensation projected to LiDAR vs LiDAR only.
Temporal improving segmentation
Contributions:

semantic image beased object removal vs event-based (maybe faster or at least only removed the dynamic objects and leaves static in place).

Experiments:
- CARLA (not preferred, because synthetic)
- On car data in private area (GT: RTK)
- DSEC as much as possible, because it is public
- MVSEC (depends)
- SLAM map quality
- SLAM drift in static (car stays, scene moves), how to quantify without GT?
- SLAM accuracy (DSEC)
- Lidar motion seg vs event motion seg.

\begin{itemize}
    \item Event-based Motion segmentation with jointly:
    \item motion segmentation
    \item pose estimation
    \item depth estimation
    \item application in SLAM
\end{itemize}

Unknowns
\begin{itemize}
    \item Benchmarks?
    \item Data for experiments?
    \item Message?
    \item Relevance for robotics?
\end{itemize}

\begin{itemize}
    \item Week 1: dataset collection
    \item Week 1: Comparison tables for motion comp.
    \item week 2: SLAM tables
    \item week 3 writing \& finetuning paper
    \item week 3.5: video (check if due at same time)
\end{itemize}

Updates Stam 16.01.2023
\begin{itemize}
\item Improving models in training (forward, backward, flow)
\item Also checked Theseus optimization (that could improve sparse to dense flow)
\item Now: Mostly ablations
\end{itemize}

Updates Weining 16.01.2023
\begin{itemize}
\item Ablations on inputs
\item motion comp can improve about 1.6 IoU
\item Additional flow can boost about 1.6 IoU
\item Temporal can boost by about 1.1 IoU
\item Temporal gives more consistent (less jittering)
\end{itemize}

SLAM updates 16.01.2023
\begin{itemize}
\item Vision-LiDAR Projection this week
\item Dataset collection
\item Car calibration
\item Run updated model on DSEC data
\end{itemize}

Updates Stam 20.01.2023
\begin{itemize}
\item Supervision with LOAM "GT" pose
\item very close to E-RAFT performance (and E-RAFT) was trained unfair with test set as validation set
\item Transformer supposed to cross correlate temporal voxels in voxelgrid, but itdoes not work well and is abandoned
\item Over weekend the models should get fixed
\item Also checked Theseus optimization (that could improve sparse to dense flow)
\item Now: Mostly ablations
\item Hoping to get model for EV-IMO to run ablation
\end{itemize}

Updates Weining 20.01.2023
\begin{itemize}
\item Indoor samples
\item 
\end{itemize}

Updates SLAM 20.01.2023
\begin{itemize}
\item Write lidar image projection and point cloud filtering node
\item Latest DSEC models
\item Data collection
\item fix metrics for filtering
\item run SLAM w / wo event / Lidar motion filter and make 
\end{itemize}

Updates SLAM 25.01.2023
\begin{itemize}
\item Abel: Wrote lidar image projection and point cloud filtering node, works nicely
\item Abel: Writing: next week
\item Abel: Run experiments on SLAM (point cloud filtering for mapping and state estimation)
\item: Alfredo calibratoins
\item Alfredo: feature tracking metrics
\item Alfredo: WIl put motion segmentation depth ourput in bagfile
\end{itemize}

Updates Stam 25.01.2023
\begin{itemize}
\item Running model (Only RNN is missing)
\item EV-IMO training started
\item Started comparisons with EV-IMO
\item Some nice-to-have in the pipeline on architectures if there is time
\item Now working on some writing, collecting videos
\end{itemize}

Updates Weining 25.01.2023
\begin{itemize}
\item DSEC annotations of test set masks
\item setup comparison of EV-IMO
\item DSEC flow submission to leaderboard

\end{itemize}

Updates SLAM 27.01.2023
\begin{itemize}
\item Abel, add depth channel from motion segmentation and hallucinate dynamic objects overlayed on lidar data
\item Abel, run experiments and visualization Mon-Wed
\item Abel, Thur & Fri writing, cutting video
\item Alfredo: Data collection and feature metrics
\end{itemize}

Updates motion segmentation 27.01.2023
\begin{itemize}
\item Stam: Produced best number (35 IoU) from competing method, far worse than ours
\item Stam: Some debugging
\item Stam: Can add some discussion on things tried, e.g. architecture and what effect it has
\item Weining makes videos and figures (mostly EV-IMO)
\end{itemize}

Updates SLAM 01.02.2023
\begin{itemize}
\item Abel: Ready for experiments, need data (DAVIS, DSEC, Robosense)
\item Abel: will write also from today in parallel to running stuff
\item Abel: Record beamsplitter data indoor / outdoor
\item Abel: Friday only writing
\item Alfredo: Feature statistics finish today
\item Alfredo: Lidar calibration
\item Alfredo: More interlaken sequences
\end{itemize}

Updates motion segmentation 01.02.2023
\begin{itemize}
\item Stam: Removing augmentations at end of training  hugely improves flow model
\item Stam: Focus on writing
\item Weining: Focus on figures
\item Possibly add gifs
\item Weining: has almost all numbers generated

\end{itemize}
